Adaptive Representations for Tracking Breaking News on Twitter

Twitter is often the most up-to-date source for finding and tracking breaking news stories. Therefore, there is considerable interest in developing filters for tweet streams in order to track and summarize stories. This is a non-trivial text analytics task as tweets are short, and standard retrieval methods often fail as stories evolve over time. In this paper we examine the effectiveness of adaptive mechanisms for tracking and summarizing breaking news stories. We evaluate the effectiveness of these mechanisms on a number of recent news events for which manually curated timelines are available. Assessments based on ROUGE metrics indicate that an adaptive approaches are best suited for tracking evolving stories on Twitter.

==> figures/fig_batkid.tex <==
  \begin{scope}[shift={(50.0,0)}]
    \begin{scope}[shift={(0,130.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text11) {};
    \end{scope}
    \begin{scope}[shift={(0,118.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text17) {};
    \end{scope}
    \begin{scope}[shift={(0,106.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text23) {};
    \end{scope}
    \begin{scope}[shift={(0,94.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text29) {};
    \end{scope}
    \begin{scope}[shift={(0,82.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text35) {};
    \end{scope}
    \begin{scope}[shift={(0,70.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text41) {};
    \end{scope}
    \begin{scope}[shift={(0,58.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text47) {};
    \end{scope}
    \begin{scope}[shift={(0,46.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text53) {};
    \end{scope}
    \begin{scope}[shift={(0,34.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text59) {};
    \end{scope}
    \begin{scope}[shift={(0,22.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text65) {};
    \end{scope}
    \begin{scope}[shift={(0,10.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text71) {};
    \end{scope}
    \path (0.0000,10.0000) -- (0.0000,10.0000) -- (0.0000,130.0000) --
      (0.0000,130.0000);
  \end{scope}
  \begin{scope}[shift={(50.0,0)}]
    \begin{scope}[shift={(0,130.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text81) {0.0};
    \end{scope}
    \begin{scope}[shift={(0,118.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text87) {0.1};
    \end{scope}
    \begin{scope}[shift={(0,106.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text93) {0.2};
    \end{scope}
    \begin{scope}[shift={(0,94.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text99) {0.3};
    \end{scope}
    \begin{scope}[shift={(0,82.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text105) {0.4};
    \end{scope}
    \begin{scope}[shift={(0,70.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text111) {0.5};
    \end{scope}
    \begin{scope}[shift={(0,58.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text117) {0.6};
    \end{scope}
    \begin{scope}[shift={(0,46.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text123) {0.7};
    \end{scope}
    \begin{scope}[shift={(0,34.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text129) {0.8};
    \end{scope}
    \begin{scope}[shift={(0,22.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text135) {0.9};
    \end{scope}
    \begin{scope}[shift={(0,10.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text141) {1.0};
    \end{scope}
    \path[draw=black] (-6.0000,10.0000) -- (0.0000,10.0000) -- (0.0000,130.0000) --
      (-6.0000,130.0000);
  \end{scope}
  \node[left] at (23.878788+-10,70) (text145) {f};
  \begin{scope}[shift={(0,130.0)}]
    \begin{scope}[shift={(50.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text153) {1};
    \end{scope}
    \begin{scope}[shift={(82.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text159) {2};
    \end{scope}
    \begin{scope}[shift={(114.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text165) {3};
    \end{scope}
    \begin{scope}[shift={(146.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text171) {4};
    \end{scope}
    \begin{scope}[shift={(178.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text177) {5};
    \end{scope}
    \begin{scope}[shift={(210.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text183) {6};
    \end{scope}
    \begin{scope}[shift={(242.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text189) {7};
    \end{scope}
    \begin{scope}[shift={(274.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text195) {8};
    \end{scope}
    \begin{scope}[shift={(306.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text201) {9};
    \end{scope}
    \begin{scope}[shift={(338.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text207) {10};
    \end{scope}
    \begin{scope}[shift={(370.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text213) {};
    \end{scope}
    \path[draw=black] (50.0000,6.0000) -- (50.0000,0.0000) -- (370.0000,0.0000) --
      (370.0000,6.0000);
  \end{scope}
  \node at (210,165.87878) (text217) {Event Period};
  \path[draw=c6b94b0,opacity=0.800,line width=1.600pt] (66.0000,88.0000) --
    (98.0000,91.6000) -- (130.0000,94.0000) -- (162.0000,89.2000) --
    (194.0000,96.4000) -- (226.0000,85.6000) -- (258.0000,88.0000) --
    (290.0000,76.0000) -- (322.0000,85.6000) -- (354.0000,89.2000);
  \path[draw=cd26b5f,opacity=0.800,line width=1.600pt] (66.0000,98.8000) --
    (98.0000,91.6000) -- (130.0000,97.6000) -- (162.0000,90.4000) --
    (194.0000,103.6000) -- (226.0000,89.2000) -- (258.0000,89.2000) --
    (290.0000,109.6000) -- (322.0000,85.6000) -- (354.0000,82.0000);
  \path[draw=cd39651,opacity=0.800,line width=1.600pt] (66.0000,88.0000) --
    (98.0000,118.0000) -- (130.0000,118.0000) -- (162.0000,130.0000) --
    (194.0000,130.0000) -- (226.0000,130.0000) -- (258.0000,130.0000) --
    (290.0000,130.0000) -- (322.0000,130.0000) -- (354.0000,130.0000);

    
    \node[right] at (86,22.878788) (legend_w2vd_w24_r15_v200) {Adaptive NNLM};
    \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
      (66.0000,15.0000) rectangle (81.0000,24.0000);
    \node[right] at (86,37.878788) (legend_w2vs_w24_r15_v200) {Nonadaptive NNLM};
    \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
      (66.0000,30.0000) rectangle (81.0000,39.0000);
    \node[right] at (86,52.878788) (legend_tfidfd_w24_r15_v0) {Term Frequency};
    \path[draw=cd39651,fill=cfdb462,opacity=0.800,rounded corners=0.0000cm]
      (66.0000,45.0000) rectangle (81.0000,54.0000);



==> figures/fig_fit_events.tex <==
\small
    \begin{tabu} to \columnwidth { @{\hspace{0.3em}}X[2,l] |@{\hspace{0.3em}}X[r] |@{\hspace{0.3em}}X[1.5,r] |@{\hspace{0.3em}}X[1.2,r] |@{\hspace{0.3em}}X[r] |@{\hspace{0.3em}}X[r] |@{\hspace{0.3em}}X[1.5,r] |@{\hspace{0.3em}}X[1.2,r] |@{\hspace{0.3em}}X[r] }
    
    Event:    & \multicolumn{8}{l}{ROUGE-1 Scores} \\ \hline
    ~         & \multicolumn{4}{l|@{\hspace{0.3em}}}{Recall} & \multicolumn{4}{l}{Precision} \\ \hline
    ~         & Max & \textbf{Adap.} & Static & tf    & Max & \textbf{Adap.}  & Static & tf \\ \hline
Batkid & \textbf{0.41} & \textbf{0.18} & 0.14 & 0.06 & \textbf{0.44} & 0.28 & \textbf{0.29} & 0.10 \\ \hline
Iran & \textbf{0.89} & \textbf{0.47} & 0.40 & 0.17 & \textbf{0.60} & 0.17 & \textbf{0.17} & 0.14 \\ \hline
LAX & \textbf{0.87} & \textbf{0.21} & 0.15 & 0.10 & \textbf{0.30} & \textbf{0.29} & 0.25 & 0.24 \\ \hline
RobFord & \textbf{0.56} & \textbf{0.14} & 0.11 & 0.04 & \textbf{0.43} & \textbf{0.42} & 0.39 & 0.15 \\ \hline
Tornado & \textbf{0.58} & \textbf{0.16} & 0.14 & 0.03 & \textbf{0.18} & 0.16 & \textbf{0.18} & 0.10 \\ \hline
Yale & \textbf{0.53} & \textbf{0.22} & 0.15 & 0.02 & \textbf{0.75} & \textbf{0.28} & 0.16 & 0.04 \\ 
\end{tabu}
\caption{ROUGE-1 Scores for ``Tuning'' Events}
\label{fig:paramscores1}

==> figures/fig_fit_models.tex <==
  \begin{scope}[shift={(40.0,0)}]
    \begin{scope}[shift={(0,130.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text15) {};
    \end{scope}
    \begin{scope}[shift={(0,115.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text21) {};
    \end{scope}
    \begin{scope}[shift={(0,100.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text27) {};
    \end{scope}
    \begin{scope}[shift={(0,85.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text33) {};
    \end{scope}
    \begin{scope}[shift={(0,70.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text39) {};
    \end{scope}
    \begin{scope}[shift={(0,55.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text45) {};
    \end{scope}
    \begin{scope}[shift={(0,40.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text51) {};
    \end{scope}
    \begin{scope}[shift={(0,25.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text57) {};
    \end{scope}
    \begin{scope}[shift={(0,10.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text63) {};
    \end{scope}
    \path (0.0000,10.0000) -- (0.0000,10.0000) -- (0.0000,130.0000) --
      (0.0000,130.0000);
  \end{scope}
  \begin{scope}[shift={(40.0,0)}]
    \begin{scope}[shift={(0,130.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text73) {0.00};
    \end{scope}
    \begin{scope}[shift={(0,115.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text79) {0.05};
    \end{scope}
    \begin{scope}[shift={(0,100.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text85) {0.10};
    \end{scope}
    \begin{scope}[shift={(0,85.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text91) {0.15};
    \end{scope}
    \begin{scope}[shift={(0,70.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text97) {0.20};
    \end{scope}
    \begin{scope}[shift={(0,55.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text103) {0.25};
    \end{scope}
    \begin{scope}[shift={(0,40.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text109) {0.30};
    \end{scope}
    \begin{scope}[shift={(0,25.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text115) {0.35};
    \end{scope}
    \begin{scope}[shift={(0,10.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text121) {0.40};
    \end{scope}
    \path[draw=black] (-6.0000,10.0000) -- (0.0000,10.0000) -- (0.0000,130.0000) --
      (-6.0000,130.0000);
  \end{scope}
  \node[left] at (30,-8) (text125) {F1};
  \begin{scope}[shift={(0,130.0)}]
    \begin{scope}[shift={(40.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (-4,12) (text133) {\small Average};
    \end{scope}
    \begin{scope}[shift={(85.71429,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (1,12) (text139) {\small Batkid};
    \end{scope}
    \begin{scope}[shift={(131.42857,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (5.857143,12) (text145) {\small Iran};
    \end{scope}
    \begin{scope}[shift={(177.14286,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (5.857143,12) (text151) {\small LAX};
    \end{scope}
    \begin{scope}[shift={(222.85714,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (0.0,12) (text157) {\small Rob F.};
    \end{scope}
    \begin{scope}[shift={(268.57143,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (-3,12) (text163) {\small Tornado};
    \end{scope}
    \begin{scope}[shift={(314.28571,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (3.857143,12) (text169) {\small Yale};
    \end{scope}
    \begin{scope}[shift={(360.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (0.857143,12) (text175) {};
    \end{scope}
    \path[draw=black] (40.0000,6.0000) -- (40.0000,0.0000) -- (360.0000,0.0000) --
      (360.0000,6.0000);
  \end{scope}
  \node at (200,162.91003) (text179) {Event / Variant};
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (228.0381,76.0000) rectangle (239.0095,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (90.8952,76.0000) rectangle (101.8667,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (136.6095,67.0000) rectangle (147.5810,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (182.3238,70.0000) rectangle (193.2952,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (273.7524,94.0000) rectangle (284.7238,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (319.4667,70.0000) rectangle (330.4381,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (45.1810,76.0000) rectangle (56.1524,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (57.3714,88.0000) rectangle (68.3429,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (331.6571,91.0000) rectangle (342.6286,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (285.9429,94.0000) rectangle (296.9143,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (103.0857,85.0000) rectangle (114.0571,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (240.2286,85.0000) rectangle (251.2000,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (194.5143,85.0000) rectangle (205.4857,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (148.8000,73.0000) rectangle (159.7714,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (160.9905,94.0000) rectangle (171.9619,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (69.5619,112.0000) rectangle (80.5333,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (343.8476,124.0000) rectangle (354.8191,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (298.1333,118.0000) rectangle (309.1048,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (252.4190,112.0000) rectangle (263.3905,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (206.7048,100.0000) rectangle (217.6762,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (115.2762,112.0000) rectangle (126.2476,130.0000);
    \node[right] at (89,17.878788) (legend_w2vd_w24_r15_v200_rsf) {Adaptive NNLM};
    \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
      (69.0000,10.0000) rectangle (84.0000,19.0000);
    \node[right] at (89,32.878788) (legend_w2vs_w24_r15_v200_rsf) {Nonadaptive
      NNLM};
    \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
      (69.0000,25.0000) rectangle (84.0000,34.0000);
    \node[right] at (89,47.878788) (legend_tfidfd_w24_r15_v0_sf) {Term Frequency};
    \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
      (69.0000,40.0000) rectangle (84.0000,49.0000);

==> figures/fig_heatmap2.tex <==
\begin{scope}% g19
\end{scope}
\begin{scope}% g21
  % path23
  \path[draw=cC0C0C0,line width=0.800pt] (118.0000,85.5000) -- (390.0000,85.5000);

  % path25
  \path[draw=cC0C0C0,line width=0.800pt] (118.0000,126.5000) -- (390.0000,126.5000);

  % path27
  \path[draw=cC0C0C0,line width=0.800pt] (118.0000,166.5000) -- (390.0000,166.5000);

  % path29
  \path[draw=cC0C0C0,line width=0.800pt] (118.0000,207.5000) -- (390.0000,207.5000);

  % path31
  \path[draw=cC0C0C0,line width=0.800pt] (118.0000,247.5000) -- (390.0000,247.5000);

  % path33
  \path[draw=cC0C0C0,line width=0.800pt] (118.0000,288.5000) -- (390.0000,288.5000);

  % path35
  \path[draw=cC0C0C0,line width=0.800pt] (118.0000,328.5000) -- (390.0000,328.5000);

  % path37
  \path[draw=cC0C0C0,line width=0.800pt] (118.0000,44.5000) -- (390.0000,44.5000);

\end{scope}
\begin{scope}% g39
  % path41
  \path[draw=cC0D0E0,line width=0.800pt] (208.5000,328.0000) -- (208.5000,338.0000);

  % path43
  \path[draw=cC0D0E0,line width=0.800pt] (253.5000,328.0000) -- (253.5000,338.0000);

  % path45
  \path[draw=cC0D0E0,line width=0.800pt] (298.5000,328.0000) -- (298.5000,338.0000);

  % path47
  \path[draw=cC0D0E0,line width=0.800pt] (344.5000,328.0000) -- (344.5000,338.0000);

  % path49
  \path[draw=cC0D0E0,line width=0.800pt] (390.5000,328.0000) -- (390.5000,338.0000);

  % path51
  \path[draw=cC0D0E0,line width=0.800pt] (162.5000,328.0000) -- (162.5000,338.0000);

  % path53
  \path[draw=cC0D0E0,line width=0.800pt] (117.5000,328.0000) -- (117.5000,338.0000);

  % path55
  \path[draw=cC0D0E0,line width=0.800pt] (118.0000,328.5000) -- (390.0000,328.5000);

\end{scope}
\begin{scope}% g61
  \begin{scope}[shift={(118.0,45.0)},scale=1.000]% g63
    % path65
    \path[fill=c1e6823] (0.0000,0.0000) -- (45.0000,0.0000) -- (45.0000,40.0000) -- (0.0000,40.0000) -- cycle;

    % path67
    \path[fill=c8cc665] (0.0000,40.0000) -- (45.0000,40.0000) -- (45.0000,81.0000) -- (0.0000,81.0000) -- cycle;

    % path69
    \path[fill=cd6e685] (0.0000,81.0000) -- (45.0000,81.0000) -- (45.0000,121.0000) -- (0.0000,121.0000) -- cycle;

    % path71
    \path[fill=c8cc665] (0.0000,121.0000) -- (45.0000,121.0000) -- (45.0000,162.0000) -- (0.0000,162.0000) -- cycle;

    % path73
    \path[fill=cd6e685] (0.0000,162.0000) -- (45.0000,162.0000) -- (45.0000,202.0000) -- (0.0000,202.0000) -- cycle;

    % path75
    \path[fill=cd6e685] (0.0000,202.0000) -- (45.0000,202.0000) -- (45.0000,243.0000) -- (0.0000,243.0000) -- cycle;

    % path77
    \path[fill=ceee] (0.0000,243.0000) -- (45.0000,243.0000) -- (45.0000,283.0000) -- (0.0000,283.0000) -- cycle;

    % path79
    \path[fill=c1e6823] (45.0000,0.0000) -- (91.0000,0.0000) -- (91.0000,40.0000) -- (45.0000,40.0000) -- cycle;

    % path81
    \path[fill=cd6e685] (45.0000,40.0000) -- (91.0000,40.0000) -- (91.0000,81.0000) -- (45.0000,81.0000) -- cycle;

    % path83
    \path[fill=c8cc665] (45.0000,81.0000) -- (91.0000,81.0000) -- (91.0000,121.0000) -- (45.0000,121.0000) -- cycle;

    % path85
    \path[fill=cd6e685] (45.0000,121.0000) -- (91.0000,121.0000) -- (91.0000,162.0000) -- (45.0000,162.0000) -- cycle;

    % path87
    \path[fill=ceee] (45.0000,162.0000) -- (91.0000,162.0000) -- (91.0000,202.0000) -- (45.0000,202.0000) -- cycle;

    % path89
    \path[fill=ceee] (45.0000,202.0000) -- (91.0000,202.0000) -- (91.0000,243.0000) -- (45.0000,243.0000) -- cycle;

    % path91
    \path[fill=ceee] (45.0000,243.0000) -- (91.0000,243.0000) -- (91.0000,283.0000) -- (45.0000,283.0000) -- cycle;

    % path93
    \path[fill=c8cc665] (91.0000,0.0000) -- (136.0000,0.0000) -- (136.0000,40.0000) -- (91.0000,40.0000) -- cycle;

    % path95
    \path[fill=c44a340] (91.0000,40.0000) -- (136.0000,40.0000) -- (136.0000,81.0000) -- (91.0000,81.0000) -- cycle;

    % path97
    \path[fill=cd6e685] (91.0000,81.0000) -- (136.0000,81.0000) -- (136.0000,121.0000) -- (91.0000,121.0000) -- cycle;

    % path99
    \path[fill=cd6e685] (91.0000,121.0000) -- (136.0000,121.0000) -- (136.0000,162.0000) -- (91.0000,162.0000) -- cycle;

    % path101
    \path[fill=c8cc665] (91.0000,162.0000) -- (136.0000,162.0000) -- (136.0000,202.0000) -- (91.0000,202.0000) -- cycle;

    % path103
    \path[fill=ceee] (91.0000,202.0000) -- (136.0000,202.0000) -- (136.0000,243.0000) -- (91.0000,243.0000) -- cycle;

    % path105
    \path[fill=cd6e685] (91.0000,243.0000) -- (136.0000,243.0000) -- (136.0000,283.0000) -- (91.0000,283.0000) -- cycle;

    % path107
    \path[fill=c1e6823] (136.0000,0.0000) -- (181.0000,0.0000) -- (181.0000,40.0000) -- (136.0000,40.0000) -- cycle;

    % path109
    \path[fill=cd6e685] (136.0000,40.0000) -- (181.0000,40.0000) -- (181.0000,81.0000) -- (136.0000,81.0000) -- cycle;

    % path111
    \path[fill=c8cc665] (136.0000,81.0000) -- (181.0000,81.0000) -- (181.0000,121.0000) -- (136.0000,121.0000) -- cycle;

    % path113
    \path[fill=cd6e685] (136.0000,121.0000) -- (181.0000,121.0000) -- (181.0000,162.0000) -- (136.0000,162.0000) -- cycle;

    % path115
    \path[fill=ceee] (136.0000,162.0000) -- (181.0000,162.0000) -- (181.0000,202.0000) -- (136.0000,202.0000) -- cycle;

    % path117
    \path[fill=ceee] (136.0000,202.0000) -- (181.0000,202.0000) -- (181.0000,243.0000) -- (136.0000,243.0000) -- cycle;

    % path119
    \path[fill=ceee] (136.0000,243.0000) -- (181.0000,243.0000) -- (181.0000,283.0000) -- (136.0000,283.0000) -- cycle;

    % path121
    \path[fill=c44a340] (181.0000,0.0000) -- (227.0000,0.0000) -- (227.0000,40.0000) -- (181.0000,40.0000) -- cycle;

    % path123
    \path[fill=c44a340] (181.0000,40.0000) -- (227.0000,40.0000) -- (227.0000,81.0000) -- (181.0000,81.0000) -- cycle;

    % path125
    \path[fill=cd6e685] (181.0000,81.0000) -- (227.0000,81.0000) -- (227.0000,121.0000) -- (181.0000,121.0000) -- cycle;

    % path127
    \path[fill=cd6e685] (181.0000,121.0000) -- (227.0000,121.0000) -- (227.0000,162.0000) -- (181.0000,162.0000) -- cycle;

    % path129
    \path[fill=cd6e685] (181.0000,162.0000) -- (227.0000,162.0000) -- (227.0000,202.0000) -- (181.0000,202.0000) -- cycle;

    % path131
    \path[fill=ceee] (181.0000,202.0000) -- (227.0000,202.0000) -- (227.0000,243.0000) -- (181.0000,243.0000) -- cycle;

    % path133
    \path[fill=ceee] (181.0000,243.0000) -- (227.0000,243.0000) -- (227.0000,283.0000) -- (181.0000,283.0000) -- cycle;

    % path135
    \path[fill=c44a340] (227.0000,0.0000) -- (272.0000,0.0000) -- (272.0000,40.0000) -- (227.0000,40.0000) -- cycle;

    % path137
    \path[fill=c44a340] (227.0000,40.0000) -- (272.0000,40.0000) -- (272.0000,81.0000) -- (227.0000,81.0000) -- cycle;

    % path139
    \path[fill=c8cc665] (227.0000,81.0000) -- (272.0000,81.0000) -- (272.0000,121.0000) -- (227.0000,121.0000) -- cycle;

    % path141
    \path[fill=cd6e685] (227.0000,121.0000) -- (272.0000,121.0000) -- (272.0000,162.0000) -- (227.0000,162.0000) -- cycle;

    % path143
    \path[fill=cd6e685] (227.0000,162.0000) -- (272.0000,162.0000) -- (272.0000,202.0000) -- (227.0000,202.0000) -- cycle;

    % path145
    \path[fill=ceee] (227.0000,202.0000) -- (272.0000,202.0000) -- (272.0000,243.0000) -- (227.0000,243.0000) -- cycle;

    % path147
    \path[fill=ceee] (227.0000,243.0000) -- (272.0000,243.0000) -- (272.0000,283.0000) -- (227.0000,283.0000) -- cycle;

  \end{scope}
  \begin{scope}[shift={(118.0,45.0)},scale=1.000]% g149
  \end{scope}
\end{scope}

\begin{scope}[shift={(118.0,45.0)},scale=1.000]% g155
  \begin{scope}[shift={(17.0,2.0)}]% g157
    % text159
    \path[color=black,fill=black] (3,15) node (text159) {7};

  \end{scope}
  \begin{scope}[shift={(17.0,43.0)}]% g161
    % text163
    \path[color=black,fill=black] (3,15) node (text163) {3};

  \end{scope}
  \begin{scope}[shift={(17.0,83.0)}]% g165
    % text167
    \path[color=black,fill=black] (3,15) node (text167) {1};

  \end{scope}
  \begin{scope}[shift={(17.0,124.0)}]% g169
    % text171
    \path[color=black,fill=black] (3,15) node (text171) {3};

  \end{scope}
  \begin{scope}[shift={(17.0,164.0)}]% g173
    % text175
    \path[color=black,fill=black] (3,15) node (text175) {1};

  \end{scope}
  \begin{scope}[shift={(17.0,205.0)}]% g177
    % text179
    \path[color=black,fill=black] (3,15) node (text179) {1};

  \end{scope}
  \begin{scope}[shift={(17.0,245.0)}]% g181
    % text183
    \path[color=black,fill=black] (3,15) node (text183) {0};

  \end{scope}
  \begin{scope}[shift={(62.0,2.0)}]% g185
    % text187
    \path[color=black,fill=black] (3,15) node (text187) {8};

  \end{scope}
  \begin{scope}[shift={(62.0,43.0)}]% g189
    % text191
    \path[color=black,fill=black] (3,15) node (text191) {2};

  \end{scope}
  \begin{scope}[shift={(62.0,83.0)}]% g193
    % text195
    \path[color=black,fill=black] (3,15) node (text195) {4};

  \end{scope}
  \begin{scope}[shift={(62.0,124.0)}]% g197
    % text199
    \path[color=black,fill=black] (3,15) node (text199) {2};

  \end{scope}
  \begin{scope}[shift={(62.0,164.0)}]% g201
    % text203
    \path[color=black,fill=black] (3,15) node (text203) {0};

  \end{scope}
  \begin{scope}[shift={(62.0,205.0)}]% g205
    % text207
    \path[color=black,fill=black] (3,15) node (text207) {0};

  \end{scope}
  \begin{scope}[shift={(62.0,245.0)}]% g209
    % text211
    \path[color=black,fill=black] (3,15) node (text211) {0};

  \end{scope}
  \begin{scope}[shift={(108.0,2.0)}]% g213
    % text215
    \path[color=black,fill=black] (3,15) node (text215) {4};

  \end{scope}
  \begin{scope}[shift={(108.0,43.0)}]% g217
    % text219
    \path[color=black,fill=black] (3,15) node (text219) {6};

  \end{scope}
  \begin{scope}[shift={(108.0,83.0)}]% g221
    % text223
    \path[color=black,fill=black] (3,15) node (text223) {1};

  \end{scope}
  \begin{scope}[shift={(108.0,124.0)}]% g225
    % text227
    \path[color=black,fill=black] (3,15) node (text227) {1};

  \end{scope}
  \begin{scope}[shift={(108.0,164.0)}]% g229
    % text231
    \path[color=black,fill=black] (3,15) node (text231) {3};

  \end{scope}
  \begin{scope}[shift={(108.0,205.0)}]% g233
    % text235
    \path[color=black,fill=black] (3,15) node (text235) {0};

  \end{scope}
  \begin{scope}[shift={(108.0,245.0)}]% g237
    % text239
    \path[color=black,fill=black] (3,15) node (text239) {1};

  \end{scope}
  \begin{scope}[shift={(153.0,2.0)}]% g241
    % text243
    \path[color=black,fill=black] (3,15) node (text243) {8};

  \end{scope}
  \begin{scope}[shift={(153.0,43.0)}]% g245
    % text247
    \path[color=black,fill=black] (3,15) node (text247) {2};

  \end{scope}
  \begin{scope}[shift={(153.0,83.0)}]% g249
    % text251
    \path[color=black,fill=black] (3,15) node (text251) {4};

  \end{scope}
  \begin{scope}[shift={(153.0,124.0)}]% g253
    % text255
    \path[color=black,fill=black] (3,15) node (text255) {2};

  \end{scope}
  \begin{scope}[shift={(153.0,164.0)}]% g257
    % text259
    \path[color=black,fill=black] (3,15) node (text259) {0};

  \end{scope}
  \begin{scope}[shift={(153.0,205.0)}]% g261
    % text263
    \path[color=black,fill=black] (3,15) node (text263) {0};

  \end{scope}
  \begin{scope}[shift={(153.0,245.0)}]% g265
    % text267
    \path[color=black,fill=black] (3,15) node (text267) {0};

  \end{scope}
  \begin{scope}[shift={(198.0,2.0)}]% g269
    % text271
    \path[color=black,fill=black] (3,15) node (text271) {6};

  \end{scope}
  \begin{scope}[shift={(198.0,43.0)}]% g273
    % text275
    \path[color=black,fill=black] (3,15) node (text275) {6};

  \end{scope}
  \begin{scope}[shift={(198.0,83.0)}]% g277
    % text279
    \path[color=black,fill=black] (3,15) node (text279) {1};

  \end{scope}
  \begin{scope}[shift={(198.0,124.0)}]% g281
    % text283
    \path[color=black,fill=black] (3,15) node (text283) {1};

  \end{scope}
  \begin{scope}[shift={(198.0,164.0)}]% g285
    % text287
    \path[color=black,fill=black] (3,15) node (text287) {2};

  \end{scope}
  \begin{scope}[shift={(198.0,205.0)}]% g289
    % text291
    \path[color=black,fill=black] (3,15) node (text291) {0};

  \end{scope}
  \begin{scope}[shift={(198.0,245.0)}]% g293
    % text295
    \path[color=black,fill=black] (3,15) node (text295) {0};

  \end{scope}
  \begin{scope}[shift={(244.0,2.0)}]% g297
    % text299
    \path[color=black,fill=black] (3,15) node (text299) {6};

  \end{scope}
  \begin{scope}[shift={(244.0,43.0)}]% g301
    % text303
    \path[color=black,fill=black] (3,15) node (text303) {5};

  \end{scope}
  \begin{scope}[shift={(244.0,83.0)}]% g305
    % text307
    \path[color=black,fill=black] (3,15) node (text307) {3};

  \end{scope}
  \begin{scope}[shift={(244.0,124.0)}]% g309
    % text311
    \path[color=black,fill=black] (3,15) node (text311) {1};

  \end{scope}
  \begin{scope}[shift={(244.0,164.0)}]% g313
    % text315
    \path[color=black,fill=black] (3,15) node (text315) {1};

  \end{scope}
  \begin{scope}[shift={(244.0,205.0)}]% g317
    % text319
    \path[color=black,fill=black] (3,15) node (text319) {0};

  \end{scope}
  \begin{scope}[shift={(244.0,245.0)}]% g321
    % text323
    \path[color=black,fill=black] (3,15) node (text323) {0};

  \end{scope}
\end{scope}
\begin{scope}[shift={(51.0,368.0)}]% g325
  \begin{scope}% g327
    \begin{scope}% g329
      \begin{scope}[shift={(8.0,3.0)}]% g331
        % text333
        \path[color=black,fill=black] (21,15) node[above right] (text333) {$<$ 1};

        % rect337
        \path[fill=ceee,rounded corners=0.0000cm] (0.0000,4.0000) rectangle (16.0000,16.0000);

      \end{scope}
      \begin{scope}[shift={(66.0,3.0)}]% g339
        % text341
        \path[color=black,fill=black] (21,15) node[above right] (text341) {1 - 2};

        % rect345
        \path[fill=cd6e685,rounded corners=0.0000cm] (0.0000,4.0000) rectangle (16.0000,16.0000);

      \end{scope}
      \begin{scope}[shift={(131.0,3.0)}]% g347
        % text349
        \path[color=black,fill=black] (21,15) node[above right] (text349) {3 - 4};

        % rect353
        \path[fill=c8cc665,rounded corners=0.0000cm] (0.0000,4.0000) rectangle (16.0000,16.0000);

      \end{scope}
      \begin{scope}[shift={(196.0,3.0)}]% g355
        % text357
        \path[color=black,fill=black] (21,15) node[above right] (text357) {5 - 6};

        % rect361
        \path[fill=c44a340,rounded corners=0.0000cm] (0.0000,4.0000) rectangle (16.0000,16.0000);

      \end{scope}
      \begin{scope}[shift={(261.0,3.0)}]% g363
        % text365
        \path[color=black,fill=black] (21,15) node[above right] (text365) {$>$ 7};

        % rect369
        \path[fill=c1e6823,rounded corners=0.0000cm] (0.0000,4.0000) rectangle (16.0000,16.0000);

      \end{scope}
    \end{scope}
  \end{scope}
\end{scope}
\begin{scope}% g371
  % text373
  \path[color=black,fill=black] (140.66666666666669,348) node[below] (text373) {BEwT};

  % text375
  \path[color=black,fill=black] (186.00000000000003,348) node[below] (text375) {R1};

  % text377
  \path[color=black,fill=black] (231.33333333333334,348) node[below] (text377) {R2};

  % text379
  \path[color=black,fill=black] (276.6666666666667,348) node[below] (text379) {L};

  % text381
  \path[color=black,fill=black] (321.99999999999994,348) node[below] (text381) {SU};

  % text383
  \path[color=black,fill=black] (367.3333333333333,348) node[below] (text383) {SU4};

\end{scope}
\begin{scope}% g385
  % text387
  \path[color=black,fill=black] (103,71.21428571428572) node[above left] (text387) {BM25};

  % text389
  \path[color=black,fill=black] (103,111.64285714285714) node[above left] (text389) {W2V Dynamic};

  % text393
  \path[color=black,fill=black] (103,152.07142857142858) node[above left] (text393) {RI Dynamic};

  % text397
  \path[color=black,fill=black] (103,192.5) node[above left] (text397) {RRI Dynamic};

  % text401
  \path[color=black,fill=black] (103,232.92857142857144) node[above left] (text401) {W2V Static};

  % text405
  \path[color=black,fill=black] (103,273.35714285714283) node[above left] (text405) {RI Static};

  % text409
  \path[color=black,fill=black] (103,313.7857142857143) node[above left] (text409) {RRI Static};

\end{scope}

==> figures/fig_models.tex <==
  \begin{scope}[shift={(40.0,0)}]
    \begin{scope}[shift={(0,130.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text15) {};
    \end{scope}
    \begin{scope}[shift={(0,115.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text21) {};
    \end{scope}
    \begin{scope}[shift={(0,100.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text27) {};
    \end{scope}
    \begin{scope}[shift={(0,85.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text33) {};
    \end{scope}
    \begin{scope}[shift={(0,70.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text39) {};
    \end{scope}
    \begin{scope}[shift={(0,55.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text45) {};
    \end{scope}
    \begin{scope}[shift={(0,40.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text51) {};
    \end{scope}
    \begin{scope}[shift={(0,25.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text57) {};
    \end{scope}
    \begin{scope}[shift={(0,10.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text63) {};
    \end{scope}
    \path (0.0000,10.0000) -- (0.0000,10.0000) -- (0.0000,130.0000) --
      (0.0000,130.0000);
  \end{scope}
  \begin{scope}[shift={(40.0,0)}]
    \begin{scope}[shift={(0,130.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text73) {0.00};
    \end{scope}
    \begin{scope}[shift={(0,115.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text79) {0.05};
    \end{scope}
    \begin{scope}[shift={(0,100.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text85) {0.10};
    \end{scope}
    \begin{scope}[shift={(0,85.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text91) {0.15};
    \end{scope}
    \begin{scope}[shift={(0,70.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text97) {0.20};
    \end{scope}
    \begin{scope}[shift={(0,55.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text103) {0.25};
    \end{scope}
    \begin{scope}[shift={(0,40.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text109) {0.30};
    \end{scope}
    \begin{scope}[shift={(0,25.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text115) {0.35};
    \end{scope}
    \begin{scope}[shift={(0,10.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text121) {0.40};
    \end{scope}
    \path[draw=black] (-6.0000,10.0000) -- (0.0000,10.0000) -- (0.0000,130.0000) --
      (-6.0000,130.0000);
  \end{scope}
  \node[left] at (30,-8) (text125) {F1};
  \begin{scope}[shift={(0,130.0)}]
    \begin{scope}[shift={(40.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (0,12) (text133) {Avg};
    \end{scope}
    \begin{scope}[shift={(69.09091,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text139) {1};
    \end{scope}
    \begin{scope}[shift={(98.18182,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text145) {2};
    \end{scope}
    \begin{scope}[shift={(127.27273,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text151) {3};
    \end{scope}
    \begin{scope}[shift={(156.36364,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text157) {4};
    \end{scope}
    \begin{scope}[shift={(185.45455,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text163) {5};
    \end{scope}
    \begin{scope}[shift={(214.54545,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text169) {6};
    \end{scope}
    \begin{scope}[shift={(243.63636,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text175) {7};
    \end{scope}
    \begin{scope}[shift={(272.72727,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text181) {8};
    \end{scope}
    \begin{scope}[shift={(301.81818,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text187) {9};
    \end{scope}
    \begin{scope}[shift={(330.90909,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text193) {10};
    \end{scope}
    \begin{scope}[shift={(360.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node[right] at (4.545455,12) (text199) {};
    \end{scope}
    \path[draw=black] (40.0000,6.0000) -- (40.0000,0.0000) -- (360.0000,0.0000) --
      (360.0000,6.0000);
  \end{scope}
  \node at (200,162.91003) (text203) {Event id / Variant};
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (246.9333,91.0000) rectangle (253.9151,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (72.3879,76.0000) rectangle (79.3697,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (217.8424,106.0000) rectangle (224.8242,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (276.0242,97.0000) rectangle (283.0060,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (159.6606,55.0000) rectangle (166.6424,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (130.5697,70.0000) rectangle (137.5515,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (101.4788,109.0000) rectangle (108.4606,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (305.1151,118.0000) rectangle (312.0970,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (188.7515,73.0000) rectangle (195.7333,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (334.2061,73.0000) rectangle (341.1879,130.0000);
  \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
    (43.2970,88.0000) rectangle (50.2788,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (51.0545,100.0000) rectangle (58.0364,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (341.9636,103.0000) rectangle (348.9454,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (196.5091,112.0000) rectangle (203.4909,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (312.8727,118.0000) rectangle (319.8546,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (109.2364,112.0000) rectangle (116.2182,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (138.3273,82.0000) rectangle (145.3091,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (80.1455,103.0000) rectangle (87.1273,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (254.6909,82.0000) rectangle (261.6727,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (167.4182,58.0000) rectangle (174.4000,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (283.7818,100.0000) rectangle (290.7636,130.0000);
  \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
    (225.6000,127.0000) rectangle (232.5818,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (116.9939,121.0000) rectangle (123.9758,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (233.3576,103.0000) rectangle (240.3394,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (349.7212,124.0000) rectangle (356.7030,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (204.2667,112.0000) rectangle (211.2485,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (320.6303,121.0000) rectangle (327.6121,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (58.8121,115.0000) rectangle (65.7939,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (87.9030,88.0000) rectangle (94.8848,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (175.1757,118.0000) rectangle (182.1576,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (291.5394,121.0000) rectangle (298.5212,130.0000);
  \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
    (146.0848,97.0000) rectangle (153.0667,130.0000);
    \node[right] at (89,17.878788) (legend_w2vd_w24_r15_v200_rsf) {Adaptive NNLM};
    \path[draw=c95b957,fill=cb3de69,opacity=0.800,rounded corners=0.0000cm]
      (69.0000,10.0000) rectangle (84.0000,19.0000);
    \node[right] at (89,32.878788) (legend_w2vs_w24_r15_v200_rsf) {Nonadaptive
      NNLM};
    \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
      (69.0000,25.0000) rectangle (84.0000,34.0000);
    \node[right] at (89,47.878788) (legend_tfidfd_w24_r15_v0_sf) {Term Frequency};
    \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
      (69.0000,40.0000) rectangle (84.0000,49.0000);

==> figures/fig_yale.tex <==
  \begin{scope}[shift={(50.0,0)}]
    \begin{scope}[shift={(0,130.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text11) {};
    \end{scope}
    \begin{scope}[shift={(0,118.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text17) {};
    \end{scope}
    \begin{scope}[shift={(0,106.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text23) {};
    \end{scope}
    \begin{scope}[shift={(0,94.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text29) {};
    \end{scope}
    \begin{scope}[shift={(0,82.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text35) {};
    \end{scope}
    \begin{scope}[shift={(0,70.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text41) {};
    \end{scope}
    \begin{scope}[shift={(0,58.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text47) {};
    \end{scope}
    \begin{scope}[shift={(0,46.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text53) {};
    \end{scope}
    \begin{scope}[shift={(0,34.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text59) {};
    \end{scope}
    \begin{scope}[shift={(0,22.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text65) {};
    \end{scope}
    \begin{scope}[shift={(0,10.0)}]
      \path[draw=cd3d3d3,opacity=0.800] (0.0000,0.0000) -- (320.0000,0.0000);
      \node[left] at (-3,0) (text71) {};
    \end{scope}
    \path (0.0000,10.0000) -- (0.0000,10.0000) -- (0.0000,130.0000) --
      (0.0000,130.0000);
  \end{scope}
  \begin{scope}[shift={(50.0,0)}]
    \begin{scope}[shift={(0,130.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text81) {0.0};
    \end{scope}
    \begin{scope}[shift={(0,118.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text87) {0.1};
    \end{scope}
    \begin{scope}[shift={(0,106.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text93) {0.2};
    \end{scope}
    \begin{scope}[shift={(0,94.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text99) {0.3};
    \end{scope}
    \begin{scope}[shift={(0,82.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text105) {0.4};
    \end{scope}
    \begin{scope}[shift={(0,70.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text111) {0.5};
    \end{scope}
    \begin{scope}[shift={(0,58.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text117) {0.6};
    \end{scope}
    \begin{scope}[shift={(0,46.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text123) {0.7};
    \end{scope}
    \begin{scope}[shift={(0,34.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text129) {0.8};
    \end{scope}
    \begin{scope}[shift={(0,22.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text135) {0.9};
    \end{scope}
    \begin{scope}[shift={(0,10.0)}]
      \path[draw=black] (0.0000,0.0000) -- (-6.0000,0.0000);
      \node[left] at (-9,0) (text141) {1.0};
    \end{scope}
    \path[draw=black] (-6.0000,10.0000) -- (0.0000,10.0000) -- (0.0000,130.0000) --
      (-6.0000,130.0000);
  \end{scope}
  \node[left] at (23.878788+-10,70) (text145) {f};
  \begin{scope}[shift={(0,130.0)}]
    \begin{scope}[shift={(50.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text153) {1};
    \end{scope}
    \begin{scope}[shift={(82.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text159) {2};
    \end{scope}
    \begin{scope}[shift={(114.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text165) {3};
    \end{scope}
    \begin{scope}[shift={(146.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text171) {4};
    \end{scope}
    \begin{scope}[shift={(178.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text177) {5};
    \end{scope}
    \begin{scope}[shift={(210.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text183) {6};
    \end{scope}
    \begin{scope}[shift={(242.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text189) {7};
    \end{scope}
    \begin{scope}[shift={(274.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text195) {8};
    \end{scope}
    \begin{scope}[shift={(306.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text201) {9};
    \end{scope}
    \begin{scope}[shift={(338.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text207) {10};
    \end{scope}
    \begin{scope}[shift={(370.0,0)}]
      \path[draw=black] (0.0000,0.0000) -- (0.0000,6.0000);
      \node at (16,15) (text213) {};
    \end{scope}
    \path[draw=black] (50.0000,6.0000) -- (50.0000,0.0000) -- (370.0000,0.0000) --
      (370.0000,6.0000);
  \end{scope}
  \node at (210,165.87878) (text217) {Event Period};
  \path[draw=c6b94b0,opacity=0.800,line width=1.600pt] (66.0000,128.8000) --
    (98.0000,92.8000) -- (130.0000,77.2000) -- (162.0000,68.8000) --
    (194.0000,79.6000) -- (226.0000,85.6000) -- (258.0000,106.0000) --
    (290.0000,100.0000) -- (322.0000,115.6000) -- (354.0000,120.4000);
  \path[draw=cd26b5f,opacity=0.800,line width=1.600pt] (66.0000,128.8000) --
    (98.0000,122.8000) -- (130.0000,122.8000) -- (162.0000,120.4000) --
    (194.0000,122.8000) -- (226.0000,124.0000) -- (258.0000,126.4000) --
    (290.0000,125.2000) -- (322.0000,127.6000) -- (354.0000,128.8000);
  \path[draw=cd39651,opacity=0.800,line width=1.600pt] (66.0000,94.0000) --
    (98.0000,94.0000) -- (130.0000,98.8000) -- (162.0000,130.0000) --
    (194.0000,122.8000) -- (226.0000,130.0000) -- (258.0000,130.0000) --
    (290.0000,130.0000) -- (322.0000,130.0000) -- (354.0000,102.4000);

    \node[right] at (86,22.878788) (legend_w2vd_w24_r15_v200) {Adaptive NNLM};
    \path[draw=c6b94b0,fill=c80b1d3,opacity=0.800,rounded corners=0.0000cm]
      (66.0000,15.0000) rectangle (81.0000,24.0000);
    \node[right] at (86,37.878788) (legend_w2vs_w24_r15_v200) {Nonadaptive NNLM};
    \path[draw=cd26b5f,fill=cfb8072,opacity=0.800,rounded corners=0.0000cm]
      (66.0000,30.0000) rectangle (81.0000,39.0000);
    \node[right] at (86,52.878788) (legend_tfidfd_w24_r15_v0) {Term Frequency};
    \path[draw=cd39651,fill=cfdb462,opacity=0.800,rounded corners=0.0000cm]
      (66.0000,45.0000) rectangle (81.0000,54.0000);


